Multi-fidelity aerodynamic data fusion by autoencoder transfer learning

Accurate aerodynamic prediction often relies on high-fidelity simulations; however, their prohibitive computational costs severely limit their applicability in data-driven modeling. This limitation motivates the development of multi-fidelity strategies that leverage inexpensive low-fidelity information without compromising accuracy. Addressing this challenge, this work presents a multi-fidelity deep learning framework that combines autoencoder-based transfer learning with a newly developed Multi-Split Conformal Prediction (MSCP) strategy to achieve uncertainty-aware aerodynamic data fusion under extreme data scarcity. The methodology leverages abundant Low-Fidelity (LF) data to learn a compact latent physics representation, which acts as a frozen knowledge base for a decoder that is subsequently fine-tuned using scarce HF samples. Tested on surface-pressure distributions for NACA airfoils (2D) and a transonic wing (3D) databases, the model successfully corrects LF deviations and achieves high-accuracy pressure predictions using minimal HF training data. Furthermore, the MSCP framework produces robust, actionable uncertainty bands with pointwise coverage exceeding 95%. By combining extreme data efficiency with uncertainty quantification, this work offers a scalable and reliable solution for aerodynamic regression in data-scarce environments.

==> commands.tex <==
%% Color definition
\definecolor{blue}{rgb}{0,0,1}
\definecolor{red}{rgb}{1,0,0}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\definecolor{grey}{RGB}{50,50,50}
\definecolor{redR}{RGB}{227, 47.3333, 39}
\definecolor{green}{RGB}{55, 160.3333, 85}
\definecolor{blue}{RGB}{55, 135, 192.3333}
\definecolor{yellow}{rgb}{0.9412, 0.7843, 0.0588}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Review Commands
\newcommand{\highlight}[1]{{\color{magenta}[#1]}}
% Rodrigo
%\definecolor{color_rebut}{RGB}{255, 140, 0}
\definecolor{color_rebut}{RGB}{20, 20, 255}

\newcommand{\rev}[1]{{\color{color_rebut}#1}}
\newcommand{\revr}[2]{ {\color{color_rebut} \sout{#1}} \rev{#2}}
\newcommand{\revs}[1]{{\color{color_rebut} \sout{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\endinput
